Detection and characterization of planets orbiting oscillating red-giant stars with NASA's TESS mission

Driven largely by multiple ground-based radial-velocity (RV) surveys and photometric space missions such as Kepler and K2, the discovery of new exoplanets has increased rapidly since the early 2000s. However, due to a target selection bias in favor of main-sequence stars, only a handful of transiting planets have been found orbiting evolved hosts. These planets, most of which are giants, hold important information regarding the formation and evolution of planetary systems. In this thesis, I sought to increase the sample of known giant planets orbiting red-giant stars, focusing on data from NASA's Transiting Exoplanet Survey Satellite (TESS) mission, and to improve their characterization. Specifically, I focused on close-in giant planets orbiting (preferably) oscillating low-luminosity red-giant branch (LLRGB) stars. To improve characterization, I developed a method to model planetary transits and stellar signals simultaneously, implementing Gaussian processes to model stellar granulation and the oscillations envelope in the time domain. My results show that the model enables time-domain asteroseismology, inferring the frequency of maximum oscillation amplitude, $\nu_\text{max}$, to within 1\%. The method's implementation is open-source and available to the community. Regarding the planet search, I assembled a pipeline, mostly comprised of third-party open-source software and explored a sample of $\sim$40,000 bright LLRGB stars in the southern hemisphere of TESS's field of view. The search identified four planet candidates, two of which are not currently known planets and orbit red-giant stars. Radial-velocity follow-up observations of both these candidates have tentatively confirmed their planetary nature. Finally, I also confirmed the planetary nature of an additional candidate, not part of the above sample, through RV observations.

==> chapters/characterization/app_orbits.tex <==
\chapter{Deriving Kepler's Laws from Newton's Gravitation}
\label{app:kepler_laws_from_newton}

In orbital mechanics, the motion between a planet and a star can be understood in the context of a two body problem. These two bodies, namely our star and planet, are treated as two point mass objects with masses $m_1$ and $m_2$ respectively, separated by a distance $r$ from each other. From the point of view of the planet, and following Newton's universal law of gravitation, the gravitational forces acting on the planet are
%
\begin{equation}
    \bm{F} = - G \frac{m_1 m_2}{r^3}\bm{r} ,
    \label{eq:newton_gravitation_law}
\end{equation}
%
where $G = 6.67260 \times 10^{-11} \text{Nm}^2\text{kg}^{-2}$ is the universal gravitational constant, and $bm{r}$ denotes the vector in the direction from the star to the planet.
Following now Newton's second law of motion in the reference of the planet, we have
%
\begin{equation}
    \bm{F} = m_2 \bm{a} = m_2 \ddot{\bm{r}} ,
    \label{eq:newton_second_law}
\end{equation}
%
where we follow the dot notation for time derivatives so that velocity $\bm{v} = \frac{d \bm{r}}{d t} = \dot{\bm{r}}$ and acceleration $\bm{a} =  \frac{d^2\bm{r}}{dt^2} = \ddot{\bm{r}}$.
Combining Eqs.~\eqref{eq:newton_gravitation_law} and \eqref{eq:newton_second_law} gives us the equality
%
\begin{equation}
    \ddot{\bm{r}} = - G \frac{m_1}{r^3}\bm{r} .
    \label{eq:gravitational_acceleration}
\end{equation}
%
Taking the cross product of $\bm{r}$ with Eq.~\eqref{eq:gravitational_acceleration} we have
%
\begin{equation}
    \bm{r} \times \ddot{\bm{r}} = 0 ,
\end{equation}
%
and expanding now the derivative of the cross product between $\bm{r}$ and $\dot{\bm{r}}$ and applying the commutative rule we find that
%
\begin{equation}
    \frac{d}{dt} (\bm{r} \times \dot{\bm{r}}) = \dot{\bm{r}} \times \dot{\bm{r}} + \bm{r} \times \ddot{\bm{r}} = \bm{r} \times \ddot{\bm{r}} = 0 \ ,
\end{equation}
%
which when integrated gives us
%
\begin{equation}
    \bm{r} \times \dot{\bm{r}} = \bm{h} ,
    \label{eq:orbital_plane}
\end{equation}
%
where the vector $\bm{h}$ is a constant vector perpendicular to both $\bm{r}$ and $\dot{\bm{r}}$ and is the normal vector that defines the orbital plane.

Since the orbit is constrained to an orbital planet, we can transform these equations of motion to polar coordinates ($r$, $\theta$), which will simplify some calculations. The polar coordinate system has two basis vectors $\bm{e_r}$, along the radius vector and $\bm{e_theta}$, perpendicular to it, which can be represented in terms of the standard (cartesian) basis vectors $\bm{e_x}$ and $\bm{e_y}$ as
%
\begin{equation}
    \begin{split}
        \bm{e_r} &= (\cos \bm{\theta})\bm{e_x} + (\sin \bm{\theta}) \bm{e_y} , \\
        \bm{e_\theta} &= - (\sin \bm{\theta})\bm{e_x} + (\cos \bm{\theta}) \bm{e_y} .
    \end{split}
    \label{eq:polar_unit_vectors}
\end{equation}
%
The unit vector have time derivatives
%
\begin{equation}
    \begin{split}
        \dot{\bm{e_r}} &= \frac{d \bm{e_r}}{dt} = \frac{d \bm{e_r}}{d \theta} \frac{d \theta}{dt} = \dot{\theta} \bm{e_\theta} , \\
        \dot{\bm{e_\theta}} &= \frac{d \bm{e_\theta}}{dt} = \frac{d \bm{e_\theta}}{d \theta} \frac{d \theta}{dt} = - \dot{\theta} \bm{e_r} .
    \end{split}
    \label{eq:polar_time_derivatives}
\end{equation}

Representing now our previous position vector $\bm{r}$ as the vector of magnitude $r$ in the direction of the radius unit vector $\bm{e_r}$, we have the polar position and its time derivatives written as
%
\begin{align}
    \bm{r} &= r \bm{e_r} , \label{eq:polar_r_position} \\
    \begin{split}
        \dot{\bm{r}} &= \frac{dr}{dt} \bm{e_r} + r \frac{d\bm{e_r}}{dt} \\
        &= \dot{r} \bm{e_r} + r \dot{\theta} \bm{e_\theta}
    \end{split} , \label{eq:polar_r_velocity} \\
    \begin{split}
        \ddot{\bm{r}} &= \frac{d^2r}{dt^2} \bm{e_r} + \frac{dr}{dt} \frac{d\bm{e_r}}{dt} + \frac{dr}{dt} \frac{d\bm{e_r}}{dt} + r \frac{d^2\bm{e_r}}{dt^2} \\
        &= \ddot{\bm{r}} \bm{e_r} + 2 \dot{r} \dot{\theta} \bm{e_\theta} + r \ddot{\theta} \bm{e_\theta} - r \dot{\theta}^2 \bm{e_r} \\
        &= (\ddot{r} - r \dot{\theta}^2) \bm{e_r} + (r \ddot{\theta} + 2 \dot{r} \dot{\theta}) \bm{e_\theta}
    \end{split} . \label{eq:polar_r_acceleration}
\end{align}

Substituting now \eqs{\ref{eq:polar_r_acceleration}, \ref{eq:polar_r_velocity}} in \eq{\ref{eq:orbital_plane}} we get
%
\begin{equation}
    \begin{split}
        \bm{h} &= (r \bm{e_r}) \times (\dot{r} \bm{e_r} + r \dot{\theta} \bm{e_\theta}) \\
        &= r \dot{r} (\bm{e_r} \times \bm{e_r}) + r^2 \dot{\theta} (\bm{e_r} \times \bm{e_\theta}) \\
        &= r^2 \dot{\theta} \bm{e_z} \\
        &= h \bm{e_z}
    \end{split} ,
    \label{eq:angular_momentum_vector}
\end{equation}
%
where we redefined the normal vector of the orbital plane $\bm{h}$ as a vector of magnitude $h = r^2 \dot{\theta}$ and following the direction of the unit vector $\bm{e_z}$, perpendicular to the orbital plane and unit vectors $\bm{e_r}$ and $\bm{e_\theta}$.
Evaluating the area element $dA$ covered by the planet position vector $\bm{r}$ in time $dt$ as it covers an angular distance $d\theta$ is gives us
%
\begin{equation}
    \begin{split}
        \dot{A} &= \int_0^r r dr \frac{d\theta}{dt} \\
        &= \frac{1}{2} r^2 \dot{\theta} \\
        &= \frac{1}{2} h
    \end{split}
    \label{eq:kepler_second_law}
\end{equation}
%
where
%
\begin{equation}
    h = r^2 \dot{\theta}
    \label{eq:angular_h_constant}
\end{equation}
% 
is a constant.
\eq{\ref{eq:kepler_second_law}} proves that the area swept by the orbit line covers equal areas during equal intervals of time, which is Kepler's second law of planetary motion.

Using \eqs{\ref{eq:polar_r_position}}{\ref{eq:polar_r_acceleration}} in \eq{\ref{eq:gravitational_acceleration}} and considering only the vector component in the radial direction $\bm{e_r}$ gives us the differential equation
%
\begin{equation}
    \ddot{r} - r\dot{\theta}^2 = - G \frac{m_1}{r^2} .
    \label{eq:gravitational_acceleration_radial}
\end{equation}
%
Solving \eq{\ref{eq:gravitational_acceleration_radial}} can be simplified by introducing a new variable $z = \frac{1}{r}$.
For this new variable, and using \eq{\ref{eq:angular_h_constant}}, the time derivatives with respect to $r$ solve to
%
\begin{align}
    \begin{split}
        \dot{r} &= \frac{d}{dt} \left( \frac{1}{z} \right) \\
        &= \frac{d}{dz} \left( \frac{1}{z} \right) \frac{dz}{dt} \\
        &= - \frac{1}{z^2} \frac{dz}{dt} \\
        &= - \frac{1}{z^2} \frac{dz}{d\theta} \frac{d\theta}{dt} \\
        &= - \frac{1}{z^2} \frac{dz}{d\theta} \frac{h}{r^2} \\
        &= -h \frac{dz}{d\theta}
    \end{split} , \label{eq:polar_z_velocity} \\
    \begin{split}
        \ddot{r} &= -h \frac{d}{dt} \left( \frac{dz}{d\theta} \right) \\
        &= -h \frac{d}{d\theta} \left( \frac{dz}{d\theta} \right) \frac{d\theta}{dt} \\
        &= -h \frac{d^2 z}{d\theta^2} \frac{h}{r^2} \\
        &= -h^2 z^2 \frac{d^2 z}{d\theta^2}
    \end{split} . \label{eq:polar_z_acceleration}
\end{align}
%
Substituting $z = \frac{1}{r}$ and \eqs{\ref{eq:polar_z_velocity}}{\ref{eq:polar_z_acceleration}} in \eq{\ref{eq:gravitational_acceleration_radial}} yields
%
\begin{equation}
    \begin{gathered}
        -h^2 z^2 \frac{d^2 z}{d\theta^2} - r \left( \frac{h}{r^2} \right)^2 = -G \frac{m_1}{r^2} \\
        -h^2 z^2 \frac{d^2 z}{d\theta^2} - \frac{1}{z} h^2 z^4  = -G m_1 z^2 \\
        \frac{d^2 z}{d\theta^2} + z = G \frac{m_1}{h^2}
    \end{gathered} , 
    \label{eq:binet_equation}
\end{equation}
%
which is a linear second order ordinary differential equation with a general solution:
%
\begin{equation}
    z = A \sin(\theta - \varpi) + B \cos(\theta - \varpi) + G\frac{m_1}{h^2} .
    \label{eq:binet_ode_solution}
\end{equation}
%
To solve for $A$, $B$ and $\varpi$ we rotate the polar axis so that $r$ is minimum at the arbitrary point $\theta = \varpi$, making $z$ a maximum at this point and it follows:
%
\begin{align}
    \begin{gathered} \label{eq:ode_limit_first_derivative}
        \frac{dz}{d\theta} = 0 \\
        -A \cos(\theta -\varpi) + B \sin(\theta - \varpi) = 0 \\
        -A \cos(\theta - \varpi) = 0 \\
        A = 0
    \end{gathered} , \\
    \begin{gathered} \label{eq:ode_limit_second_derivative}
        \frac{d^2z}{d\theta^2} < 0 \\
        -A \sin(\theta - \varpi) - B \cos(\theta - \varpi) < 0 \\
        -B < 0 \\
        B > 0
    \end{gathered} .
\end{align}
%
Plugging these expressions into \eq{\ref{eq:binet_ode_solution}} along with $z = \frac{1}{r}$ results in
%
\begin{equation}
    \begin{split}
        z &= B \cos(\theta - \varpi) + \frac{Gm_1}{h^2} \\
        r &= \frac{\frac{h^2}{Gm_1}}{1 + \frac{Bh^2}{Gm_1} \cos(\theta - \varpi)} \\
        r &= \frac{p}{1 + e \cos(\theta - \varpi)}
    \end{split} .
    \label{eq:conic_curves}
\end{equation}
%
\eq{\ref{eq:conic_curves}} is the equation for conics, which are the sets of curves obtained from the intersection of a surface of a cone with a plane, where $e = \frac{Bh^2}{Gm_1}$ is the \textit{eccentricity} and
\begin{equation}
    p = \frac{h^2}{Gm_1}
    \label{eq:p_h_relation}
\end{equation}
%
is called the \textit{semi-latus rectum}.
For $0 \leq e < 1$ the curves are restricted to elliptical motions and
%
\begin{equation}
    p = a(1 - e^2) ,
    \label{eq:semi_latus_rectum}
\end{equation}
%
where $a$ is the \textit{semi-major axis} of the ellipse, related to the \textit{semi-minor axis}, $b$ and the eccentricity, $e$ by
%
\begin{equation}
    b^2 = a^2(1 - e^2) .
    \label{eq:semi_minor_axis}
\end{equation}
%
\eq{\ref{eq:conic_curves}} is then written as
%
\begin{equation}
    r = \frac{a(1 - e^2)}{1 + e \cos(\theta - \varpi)} \ ,
    \label{eq:kepler_first_law_theta}
\end{equation}
%
and gives the distance $r$ from the ellipse focus (star) to the point on the ellipse (planet) for each position in the orbit defined by its angular value $\theta$.
This is Kepler's first law of planetary motion, which states that the path of planet around its star is an ellipse with the star at one focus.
The angle $\theta$, called the \textit{true longitude} evaluates to the minimum and maximum of \eq{\ref{eq:kepler_first_law_theta}} at $\theta = \varpi$ and $\theta = \varpi + \pi$, respectively. These points in the ellipse are referred to as the \textit{periapsis} and \textit{apoapsis}, respectively.
$\varpi$ is called the \textit{longitude of periapsis} as it representes the angular location of the periapsis of the ellipse with respect to the reference direction.
For the special of $e = 0$, the expression simplifies to that of a circular orbit with radius $r = a$ and $\varpi$ is undefined since all points in the orbit are now equidistant from the focus.
If we now define the \textit{true anomaly} angle $f = \theta - \varpi$ we can rewrite \eq{\ref{eq:kepler_first_law_theta}} so that the argument of the equation is the angular location from the periapsis
%
\begin{equation}
    r = \frac{a(1 - e^2)}{1 + e  \cos f} .
    \label{eq:kepler_first_law}
\end{equation}

Although \eq{\ref{eq:kepler_first_law}} has no reference to time as it is a function of $\theta$, we know from \eq{\ref{eq:kepler_second_law}} that the area swept by the orbit line covers equal areas during equal intervals of time. 
Then, for a complete orbit with period $P$, the star-planet line should cover the entire area of the ellipse $A = \pi a b$, which, together with \eqs{\ref{eq:semi_latus_rectum}}{\ref{eq:semi_minor_axis}} and $p = \frac{h^2}{Gm_1}$ we can write
%
\begin{equation}
    \begin{split}
        \frac{1}{2} h P &= \pi a b \\
        \frac{1}{4} h^2 P^2 &= \pi^2 a^2 b^2 \\
        P^2 &= \frac{4 \pi^2}{Gm_1} \frac{a^2 b^2}{p} \\
        P^2 &= \frac{4 \pi^2}{Gm_1} \frac{a^4(1 - e^2)}{a(1 - e^2)} \\
        P^2 &= \frac{4 \pi^2}{Gm_1} a^3
    \end{split} .
    \label{eq:kepler_third_law}
\end{equation}
%
This is Kepler's third law of planetary motion, which states that period of the orbit is independent of the eccentricity $e$ and depends only on the sum of masses and the semi-major axis $a$.

We can additionally define the \textit{mean motion}, $n$ of the planet as
%
\begin{equation}
    n = \frac{2\pi}{P}
\end{equation}
%
and derive the useful expression
%
\begin{equation}
    \begin{split}
        n^2 &= \frac{4\pi^2}{P^2} \\
        n^2 &= \frac{Gm_1}{a^3} \\
        n^2 a^3 &= Gm_1
    \end{split} ,
    \label{eq:n_a_mass_relation}
\end{equation}

\eq{\ref{eq:kepler_first_law}} allows us to determine the position of the planet on the elliptical orbit given the angular position $\theta$, but we don't still have an expression for $r$ dependent on time.
To do so, we derive one by finding an expression for $\dot{r}$ in terms of $r$.
We start by deriving an equation for the magnitude of the velocity squared $v^2$.
Since $\varpi$ is a constant, $\dot{f} = \dot{\theta}$ and from \eq{\ref{eq:polar_r_velocity}} we have
%
\begin{equation}
    v^2 = \dot{\bm{r}} \cdot \dot{\bm{r}} = \dot{r}^2 + r^2 \dot{\theta}^2 = \dot{r}^2 + r^2 \dot{f}^2 .
    \label{eq:velocity_squared}
\end{equation}
%
To find expressions for $\dot{r}$ and $r\dot{f}$ we follow
%
\begin{equation}
    \begin{alignedat}{3}
        r \dot{f} &= r \dot{\theta} && \\
        &= \sqrt{r^2 \dot{\theta}^2}  && \\
        &= \sqrt{\frac{h^2}{r^2}} &&\qquad \text{from \eq{\ref{eq:angular_h_constant}}} \\
        &= \sqrt{\frac{p Gm_1}{r^2}} &&\qquad \text{from \eq{\ref{eq:p_h_relation}}} \\
        &= \sqrt{\frac{a(1 - e^2) n^2 a^3}{r^2}} &&\qquad \text{from \eqs{\ref{eq:semi_latus_rectum}}{\ref{eq:n_a_mass_relation}}} \\
        &= \sqrt{a^4 n^2 (1 - e^2) \frac{(1 + e \cos f)^2}{a^2(1 - e^2)^2}} &&\qquad \text{from \eq{\ref{eq:kepler_first_law}}} \\
        &= \sqrt{\frac{a^2 n^2 (1 + e \cos f)^2}{1 - e^2}} && \\
        &= \frac{a n}{\sqrt{1 - e^2}} (1 + e \cos f) &&
    \end{alignedat} ,
    \label{eq:r_dotf}
\end{equation}
%
and then differentiate \eq{\ref{eq:kepler_first_law}} with respect to time which gives
%
\begin{equation}
    \begin{alignedat}{3}
        \dot{r} &= \frac{d}{dt} \left( \frac{a(1 - e^2)}{1 + e  \cos f} \right) &&\qquad \text{from \eq{\ref{eq:kepler_first_law}}}\\
        &= a(1 - e^2) \frac{d}{df} \left( \frac{1}{1 + e  \cos f} \right) \frac{df}{dt} && \\
        &= a(1 - e^2) \frac{e \sin f}{(1 + e \cos f)^2} \dot{f} && \\
        &= \frac{a(1 - e^2)}{1 + e \cos f} \frac{\dot{f} e \sin f}{1 + e \cos f} && \\
        &= \frac{r \dot{f} e \sin f}{1 + e \cos f} &&\qquad \text{from \eq{\ref{eq:kepler_first_law}}} \\
        &= \frac{a n}{\sqrt{1 - e^2}} (1 + e \cos f) \frac{e \sin f}{1 + e \cos f} &&\qquad \text{from \eq{\ref{eq:r_dotf}}} \\
        &= \frac{a n}{\sqrt{1 - e^2}} e \sin f &&
    \end{alignedat} .
    \label{eq:r_dot}
\end{equation}
%
Going back to \eq{\ref{eq:velocity_squared}}, we now write
%
\begin{equation}
    \begin{alignedat}{3}
        v^2 &= \frac{a^2 n^2}{1 - e^2} (e \sin f)^2 + \frac{a^2 n^2}{1 - e^2} (1 + e \cos f)^2 &&\qquad \text{from \eqs{\ref{eq:r_dotf}}{\ref{eq:r_dot}}} \\
        &= \frac{a^2 n^2}{1 - e^2} (1 + 2e \cos f + e^2 \cos^2 f + e^2 \sin^2 f) && \\
        &= \frac{a^2 n^2}{1 - e^2} (1 + 2e \cos f + e^2) &&
    \end{alignedat} ,
    \label{eq:v_dependence_f}
\end{equation}
%
which shows the dependence of $v$ on $f$.
To show the dependence of $v$ on $r$ we further modify \eq{\ref{eq:v_dependence_f}}
%
\begin{equation}
    \begin{alignedat}{3}
        v^2 &= \frac{a^2 n^2}{1 - e^2} (2 + 2e \cos f + e^2 - 1) && \\
        &= \frac{Gm_1}{a(1 - e^2)} (2 + 2e \cos f + e^2 - 1) &&\qquad \text{from \eq{\ref{eq:n_a_mass_relation}}} \\
        &= Gm_1 \frac{2(1 + e\cos f) - (1 - e^2)}{a((1 - e^2))} && \\
        &= Gm_1 \left( \frac{2}{r} - \frac{1}{a} \right) &&\qquad \text{from \eq{\ref{eq:kepler_first_law}}}
    \end{alignedat} ,
    \label{eq:v_dependence_r}
\end{equation}
%
Finally, we return to \eq{\ref{eq:velocity_squared}} and write it with respect to $\dot{r}^2$ as
%
\begin{equation}
    \begin{alignedat}{3}
        \dot{r}^2 &= v^2 - r^2 \dot{f}^2 && \\
        &= Gm_1 \left( \frac{2}{r} - \frac{1}{a} \right) - \frac{n^2 a^2}{1 - e^2}(1 + e \cos f)^2 &&\qquad \text{from \eqs{\ref{eq:v_dependence_r}}{\ref{eq:r_dotf}}} \\
        &= n^2 a^3 \left( \frac{2}{r} - \frac{1}{a} \right) - \frac{n^2 a^2 (1 - e^2)}{r^2} &&\qquad \text{from \eqs{\ref{eq:n_a_mass_relation}}{\ref{eq:kepler_first_law}}} \\
        &= \frac{n^2 a^2}{r^2} \left[ r^2 a \left( \frac{2}{r} - \frac{1}{a} \right) \right] - a^2(1 - e^2) && \\
        &= \frac{n^2 a^2}{r^2} \left( 2ra - r^2 - a^2 + a^2 e^2 \right) && \\
        &= \frac{n^2 a^2}{r^2} \left( a^2 e^2 - (r - a)^2 \right) &&
    \end{alignedat} ,
    \label{eq:r_dot_squared_dependence_r}
\end{equation}
%
from which we can obtain
%
\begin{equation}
    \dot{r} = \frac{n a}{r} \sqrt{a^2 e^2 - (r - a)^2} ,
    \label{eq:r_dot_dependence_r}
\end{equation}

% \todo{Should probably add the derivation and figure to show where $E$ is coming from}. To solve this differential equation, we introduce the \textit{eccentric anomaly}, $E$, by modifying \eq{\ref{eq:kepler_first_law}} to 
%
\begin{equation}
    r = a(1 - e\cos E)
    \label{eq:ecc_anomaly}
\end{equation}
%
which we derive with respect to time as
%
\begin{equation}
    \begin{alignedat}{3}
        \dot{r} &= \frac{d}{dt} \left( a(1 - e\cos E) \right) && \\
        \dot{r} &= \frac{d}{dE} \left( a(1 - e\cos E) \right) \frac{dE}{dt} && \\
        \dot{r} &= a e \sin E \dot{E} &&
    \end{alignedat}
\end{equation}
%
and then compare with \eq{\ref{eq:r_dot_dependence_r}}
%
\begin{equation}
    \begin{alignedat}{3}
        a e \sin E \dot{E} &= \frac{n a}{r} \sqrt{a^2 e^2 - (r - a)^2} && \\
        a e \sin E \dot{E} &= \frac{n}{1 - e\cos E} \sqrt{a^2 e^2 - (a(1 - e \cos E) - a)^2} &&\qquad \text{from \eq{\ref{eq:ecc_anomaly}}} \\
        a e \sin E \dot{E} &= \frac{n}{1 - e\cos E} \sqrt{a^2 e^2 - a^2 e^2 \cos^2 E} && \\
        a e \sin E \dot{E} &= \frac{n}{1 - e\cos E} \sqrt{a^2 e^2 \sin^2 E} && \\
        \dot{E} &= \frac{n}{1 - e\cos E} && \\
        (1 - e\cos E) \dot{E} &= n && \\
    \end{alignedat} ,
    \label{eq:ecc_anomaly_time_derivative}
\end{equation}
%
to get the equation for the time derivative of $E$, which we then integrate in time to get the solution
%
\begin{equation}
    \begin{split}
        \int (1 - e \cos E) \frac{dE}{dt} dt  &= \int n dt \\
        \int 1 dE - \int e \cos E dE &= \int n dt \\
        E - e \sin E = nt + c
    \end{split} .
    \label{eq:ecc_time_integration}
\end{equation}
%
Defining the time $t = t_0$ as the \textit{time of periapsis passage}, for which $E = 0$, we find that $c = nt_0$ and
%
\begin{equation}
    E - e \sin E = n(t - t_0) .
    \label{eq:ecc_time}
\end{equation}
%
Finally, we define the \textit{mean anomaly}, $M$, as
%
\begin{equation}
    M = n(t - t_0) ,
    \label{eq:mean_anomaly}
\end{equation}
%
an angle which has no simple geometrical interpretation but that increases linearly with time.
%
Rewriting \eq{\ref{eq:ecc_time}} with $M$ yields
%
\begin{equation}
    M = E - e \sin E ,
    \label{eq:kepler_equation}
\end{equation}
%
which is Kepler's equation and the final equation needed to obtain the location of the planet in the orbit at any time, $t$.
To do so, we first need to define two parameters related to the dimensions of the orbit: the semi-major axis, $a$ and the eccentricity, $e$ and two related to orientations: the longitude of periapsis, $\varpi$ and the time of periapsis passage, $t_0$.
With the orbital parameters defined, we find the location of the planet in the orbit at any time $t$ by:
%
\begin{itemize}[noitemsep, topsep=1ex]
    \item Finding $M$ using \eq{\ref{eq:mean_anomaly}},
    \item Finding $E$ by solving Kepler's equation \eqalt{\ref{eq:kepler_equation}},
    \item Finding the distance $r$ using \eq{\ref{eq:ecc_anomaly}},
    \item Finding $f$ using \eq{\ref{eq:kepler_first_law}}.
\end{itemize}
%
During the orbit we have then $M = E = f = 0$ at $t = t_0$ or $t = t_0 + P$, when the orbit is at periapsis and $M = E = f = \pi$ at $t = t_0 + \frac{P}{2}$, when the orbit is at apoapsis.



==> chapters/characterization/app_quadratic_ld.tex <==
\chapter{Quadratic Limb-darkening}
\label{app:quadratic_ld}

\begin{equation}
    \lambda^e(p,z) = 
    \begin{cases}
        0, & 1 + p < z, \\
        \frac{1}{\pi} \left[ p^2 \kappa_0 + \kappa_1 - \sqrt{\frac{4 z^2 - (1 + z^2 + p^2)^2}{4}} \right], & \vert 1 - p \vert < z \leq 1 + p, \\
        p^2, & z \leq 1 - p, \\
        1, & z \leq p - 1,
    \end{cases}
    \label{eq:mandel_flux_obstruction}
\end{equation}
%
with
%
\begin{align}
    \kappa_0 = \cos^{-1} \left( \frac{p^2 + z^2 - 1}{2pz} \right), \\
    \kappa_1 = \cos^{-1} \left( \frac{1 - p^2 + z^2}{2z} \right),
\end{align}

The $\lambda^d$ and $\eta^d$ functions which are used depend on the the values of $p$ and $z$, as per Table ???, and their formulations follow
\begin{equation}
    \def\arraystretch{1.6}
    \begin{array}{lll}
        \lambda_1 &= \frac{1}{9 \pi \sqrt{p z}} \left\{ \left[ (1 - b)(2b + a - 3) - 3q(b - 2) \right] K(k) + 4pz (z^2 + 7p^2 - 4)E(k) - 3\frac{q}{a}\Pi \left( \frac{a-1}{a}, k \right) \right\}, \\
        \lambda_2 &= \frac{2}{9 \pi \sqrt{1-a}} \left[ (1 - 5z^2 + p^2 + q^2) K(k^{-1}) + (1-a)(z^2 + 7p^2 - 4)E(k^{-1}) - 3\frac{q}{a}\Pi \left( \frac{a-b}{a}, k^{-1} \right) \right], \\
        \lambda_3 &= \frac{1}{3} + \frac{16p}{9 \pi} (2p^2 - 1) E\left( \frac{1}{2k} \right) - \frac{(1 - 4p^2)(3 - 8p^2)}{9 \pi p} K\left( \frac{1}{2k} \right), \\
        \lambda_4 &= \frac{1}{3} + \frac{2}{9 \pi} \left[ 4(2p^2 - 1) E(2k) + (1 - 4p^2) K(2k) \right], \\
        \lambda_5 &= \frac{2}{3 \pi} \cos^{-1} (1 - 2p) - \frac{4}{9 \pi} (3 + 2p - 8p^2), \\
        \lambda_6 &= - \frac{2}{3} (1 - p^2)^{3/2}, \\
        \eta_1 &= (2 \pi)^{-1} \left[ \kappa_1 + 2 \eta_2 \kappa_0 - \frac{1}{4} (1 + 5p^2 + z^2) \sqrt{(1 - a)(b - 1)} \right], \\
        \eta_2 &= \frac{p^2}{2} (p^2 + 2z^2),
    \end{array}
    \label{eq:quadratic_lambda_eta_functions}
\end{equation}

\begin{table}
    \centering
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{24pt}
    \begin{tabular}{c c c c}
        \hline
        $p$ & $z$ & $\lambda^d(z)$ & $\eta^d(z)$ \\
        \hline
        (0, $\infty$) & [1 + $p$, $\infty$) & 0 & 0 \\
        0 & [0, $\infty$) & 0 & 0 \\
        (0, $\infty$) & ($\frac{1}{2}$ + $\vert p$ - $\frac{1}{2}$, 1 + $p$) & $\lambda_1$ & $\eta_1$ \\
        (0, $\frac{1}{2}$) & ($p$, 1 - $p$) & $\lambda_2$ & $\eta_2$ \\
        (0, $\frac{1}{2}$) & 1 - $p$ & $\lambda_5$ & $\eta_2$ \\
        (0, $\frac{1}{2}$) & $p$ & $\lambda_4$ & $\eta_2$ \\
        $\frac{1}{2}$ & $\frac{1}{2}$ & $\frac{1}{3}$ - $\frac{4}{9} \pi$ & $\frac{3}{32}$ \\
        ($\frac{1}{2}$, $\infty$) & $p$ & $\lambda_3$ & $\eta_1$ \\
        ($\frac{1}{2}$, $\infty$) & [$\vert$1 - $p \vert$, $p$) & $\lambda_1$ & $\eta_1$ \\
        (0, 1) & (0, $\frac{1}{2}$ - $\vert p$ - $\frac{1}{2} \vert$) & $\lambda_2$ & $\eta_2$ \\
        (0, 1) & 0 & $\lambda_6$ & $\eta_2$ \\
        (1, $\infty$) & [0, $p$ - 1) & 1 & 1 \\
        \hline
    \end{tabular}
    \caption{Selection criteria for the $\lambda^d$ and $\eta^d$ functions to use in Eq.~\eqref{eq:mandel_flux} depending on the values of $p$ and $z$. The expressions for the functions themselves are shown in Eqs.~\eqref{eq:quadratic_lambda_eta_functions}.}
    \label{tab:quadratic_lambda_eta_selection}
\end{table}


